A Proposed Forward Silicon Tracker for the Future Electron-Ion Collider and Associated Physics Studies

The future Electron-Ion Collider (EIC) will explore several fundamental questions in a broad Bjorken-x ($x_{BJ}$) and $Q^{2}$ phase space. Heavy flavor and jet products are ideal probes to precisely study the tomography of nucleon/nuclei structure, help solve the proton spin puzzle and understand the hadronizaton processes in vacuum or in the QCD medium. Due to the asymmetric collisions at the EIC, most of the final state hadrons are produced in the nucleon/nuclei beam going (forward) direction. A silicon vertex/tracking is critical to precisely measure these forward hadrons at the EIC. Details of different conceptual designs of the proposed Forward Silicon Tracker (FST) and the relevant detector performance are presented in this technical note. The associated heavy flavor and jet studies with the evaluated FST performance are discussed as well.

==> section/Fun4AllSim/Eff.tex <==
\subsection{Tracking Efficiency}
The tracking efficiency is plotted as function of $p_T$ as shown in Figure~[]. A $3\sigma$ cut is applied on the relative difference between the reconstructed and input (true) momenta.
